Beyond Accuracy: An Empirical Study of Uncertainty Estimation in Imputation

Handling missing data is a central challenge in data-driven analysis. Modern imputation methods not only aim for accurate reconstruction but also differ in how they represent and quantify uncertainty. Yet, the reliability and calibration of these uncertainty estimates remain poorly understood. This paper presents a systematic empirical study of uncertainty in imputation, comparing representative methods from three major families: statistical (MICE, SoftImpute), distribution alignment (OT-Impute), and deep generative (GAIN, MIWAE, TabCSDI). Experiments span multiple datasets, missingness mechanisms (MCAR, MAR, MNAR), and missingness rates. Uncertainty is estimated through three complementary routes: multi-run variability, conditional sampling, and predictive-distribution modeling, and evaluated using calibration curves and the Expected Calibration Error (ECE). Results show that accuracy and calibration are often misaligned: models with high reconstruction accuracy do not necessarily yield reliable uncertainty. We analyze method-specific trade-offs among accuracy, calibration, and runtime, identify stable configurations, and offer guidelines for selecting uncertainty-aware imputers in data cleaning and downstream machine learning pipelines.

==> ieee_references_all.tex <==
\begin{thebibliography}{00}
% Error processing entry 0: 'NoneType' object has no attribute 'group'
\bibitem{shapley1953value} Shapley, Lloyd S., "A Value for n-Person Games," Contributions to the Theory of Games, vol. 2, pp. 307--317, 1953.
\bibitem{banzhaf1964weighted} Banzhaf, John F., "Weighted voting doesn't work: A mathematical analysis," Rutgers Law Review, vol. 19, no. 2, pp. 317--343, 1964.
\bibitem{kalai1987weighted} Kalai, Ehud, Samet, Dov, "Weighted Shapley values," Journal of Economic Theory, vol. 36, no. 2, pp. 267--276, 1985.
\bibitem{roth1988shapley} Roth, Alvin E., "The Shapley Value: Essays in Honor of Lloyd S. Shapley," Cambridge University Press, 1988.
\bibitem{kara2024shapley} Kara, Ahmet, Olteanu, Dan, Suciu, Dan, "From Shapley Value to Model Counting and Back," Proceedings of the ACM on Management of Data, vol. 2, no. 2, pp. 1--23, 2024.
\bibitem{davidson2022shapgraph} Davidson, Susan, Deutch, Daniel, Frost, Nave, Kimelfeld, Benny, Koren, Omer, Monet, Mika{\"e}l, "ShapGraph: An holistic view of explanations through provenance graphs and Shapley values," Proceedings of the 2022 International Conference on Management of Data, pp. 2373--2376, 2022.
\bibitem{bienvenu2024shapley} Bienvenu, Meghyn, Figueira, Diego, Lafourcade, Pierre, "Shapley value computation in ontology-mediated query answering," arXiv preprint arXiv:2407.20058, 2024.
\bibitem{abramovich2024banzhaf} Abramovich, Omer, Deutch, Daniel, Frost, Nave, Kara, Ahmet, Olteanu, Dan, "Banzhaf Values for Facts in Query Answering," Proceedings of the ACM on Management of Data, vol. 2, no. 3, pp. 1--26, 2024.
\bibitem{karmakar2024expected} Karmakar, Pratik, Monet, Mika{\"e}l, Senellart, Pierre, Bressan, St{\'e}phane, "Expected Shapley-like scores of boolean functions: Complexity and applications to probabilistic databases," Proceedings of the ACM on Management of Data, vol. 2, no. 2, pp. 1--26, 2024.
\bibitem{tian2022data} Tian, Yingjie, Ding, Yurong, Fu, Saiji, Liu, Dalian, "Data boundary and data pricing based on the shapley value," IEEE Access, vol. 10, pp. 14288--14300, 2022.
\bibitem{si2024counterfactual} Si, Michelle, Pei, Jian, "Counterfactual Explanation of Shapley Value in Data Coalitions," Proceedings of the VLDB Endowment, vol. 17, no. 11, pp. 3332--3345, 2024.
\bibitem{livshits2021shapley} Livshits, Ester, Bertossi, Leopoldo, Kimelfeld, Benny, Sebag, Moshe, "The Shapley value of tuples in query answering," Logical Methods in Computer Science, vol. 17, 2021.
\bibitem{deutch2022computing} Deutch, Daniel, Frost, Nave, Kimelfeld, Benny, Monet, Mika{\"e}l, "Computing the Shapley value of facts in query answering," Proceedings of the 2022 International Conference on Management of Data, pp. 1570--1583, 2022.
\bibitem{deutch2021explanations} Deutch, Daniel, Frost, Nave, Gilad, Amir, Sheffer, Oren, "Explanations for data repair through shapley values," Proceedings of the 30th ACM International Conference on Information \& Knowledge Management, pp. 362--371, 2021.
\bibitem{livshits2022shapley} Livshits, Ester, Kimelfeld, Benny, "The Shapley value of inconsistency measures for functional dependencies," Logical Methods in Computer Science, vol. 18, 2022.
\bibitem{bertossi2023shapley} Bertossi, Leopoldo, Kimelfeld, Benny, Livshits, Ester, Monet, Mika{\"e}l, "The Shapley value in database management," ACM Sigmod Record, vol. 52, no. 2, pp. 6--17, 2023.
\bibitem{sun2024shapley} Sun, Qiheng, Zhang, Jiayao, Liu, Jinfei, Xiong, Li, Pei, Jian, Ren, Kui, "Shapley Value Approximation Based on Complementary Contribution," IEEE Transactions on Knowledge and Data Engineering, 2024.
\bibitem{luo2024applications} Luo, Xuan, Pei, Jian, "Applications and computation of the Shapley value in databases and machine learning," Companion of the 2024 International Conference on Management of Data, pp. 630--635, 2024.
\bibitem{lin2024comprehensive} Lin, Hong, Wan, Shixin, Xie, Zhongle, Chen, Ke, Zhang, Meihui, Shou, Lidan, Chen, Gang, "A Comprehensive Study of Shapley Value in Data Analytics," arXiv preprint arXiv:2412.01460, 2024.
\bibitem{semiring} Green, Todd J., Karvounarakis, Grigoris, Tannen, Val, "Provenance semirings," Proceedings of the Twenty-Sixth ACM SIGMOD-SIGACT-SIGART Symposium on Principles of Database Systems, pp. 31–40, 2007.
\bibitem{semiringRevisit} Camille Bourgaux, Pierre Bourhis, Liat Peterfreund, Michael Thomazo, "Revisiting Semiring Provenance for Datalog," 2022.
\bibitem{whyHowWhere} Cheney, James, Chiticariu, Laura, Tan, Wang-chiew, \\ "Provenance in Databases: Why, How, and Where," \\Foundations and Trends in Databases, vol. 1, pp. 379-474, 2009.
\bibitem{smallestWitness} Xiao Hu, Stavros Sintos, "Finding Smallest Witnesses for Conjunctive Queries," 2024.
\bibitem{onDemand} Elhalawati, Ali, Mennicke, Stephan, Krötzsch, Markus, "An Existential Rule Framework for Computing Why-Provenance On-Demand for Datalog," 2022.
\bibitem{SAT}title={Computing the Why-Provenance for Datalog Queries via SAT Solvers}, volume={38}, url={https://ojs.aaai.org/index.php/AAAI/article/view/28914}, DOI={10.1609/aaai.v38i9.28914}, abstractNote={Explaining an answer to a Datalog query is an essential task towards Explainable AI, especially nowadays where Datalog plays a critical role in the development of ontology-based applications. A well-established approach for explaining a query answer is the so-called why-provenance, which essentially collects all the subsets of the input database that can be used to obtain that answer via some derivation process, typically represented as a proof tree. It is well known, however, that computing the why-provenance for Datalog queries is computationally expensive, and thus, very few attempts can be found in the literature. The goal of this work is to demonstrate how off-the-shelf SAT solvers can be exploited towards an efficient computation of the why-provenance for Datalog queries. Interestingly, our SAT-based approach allows us to build the why-provenance in an incremental fashion, that is, one explanation at a time, which is much more useful in a practical context than the one-shot computation of the whole set of explanations as done by existing approaches.}, number={9}, journal={Proceedings of the AAAI Conference on Artificial Intelligence}, author={Calautti, Marco and Livshits, Ester and Pieris, Andreas and Schneider, Markus}, year={2024}, month={Mar.} , "," .
\bibitem{efficientTopK} Deutch, Daniel, Gilad, Amir, Moskovitch, Yuval, "Efficient provenance tracking for datalog using top-k queries," The VLDB Journal, vol. 27, no. 2, pp. 245–269, 2018.
\bibitem{whyAndWhere} Buneman, Peter, Khanna, Sanjeev, Tan, Wang Chiew, "Why and Where: A Characterization of Data Provenance," Proceedings of the 8th International Conference on Database Theory, pp. 316–330, 2001.
\bibitem{lineage} Cui, Yingwei, Widom, Jennifer, Wiener, Janet L., "Tracing the lineage of view data in a warehousing environment," ACM Trans. Database Syst., vol. 25, no. 2, pp. 179–227, 2000.
\bibitem{foundation} Serge Abiteboul and, "Foundations of Databases," Addison-Wesley, 1995.
\bibitem{selectiveTopK} Deutch, Daniel, Gilad, Amir, Moskovitch, Yuval, "Selective provenance for datalog programs using top-k queries," Proc. VLDB Endow., vol. 8, no. 12, pp. 1394–1405, 2015.
\bibitem{shapleyAggregate} Livshits, Ester, Bertossi, Leopoldo, Kimelfeld, Benny, Sebag, Moshe, "The Shapley Value of Tuples in Query Answering," Logical Methods in Computer Science, vol. Volume 17, Issue 3, 2021.
\bibitem{shapleyQuery} Deutch, Daniel, Frost, Nave, Kimelfeld, Benny, Monet, Mika\"{e}l, "Computing the Shapley Value of Facts in Query Answering," Proceedings of the 2022 International Conference on Management of Data, pp. 1570–1583, 2022.
\bibitem{dalvi2009probabilistic} Nilesh N. Dalvi, Christopher R\'{e}, Dan Suciu, "Probabilistic databases: Diamonds in the dirt," Communications of the ACM, vol. 52, no. 7, pp. 86--94, 2009.
\bibitem{shapGraph} , "SIGMOD '22: Proceedings of the 2022 International Conference on Management of Data," Association for Computing Machinery, 2022.
\bibitem{PUG} Seokki Lee, Bertram Ludaescher, Boris Glavic, "PUG: A Framework and Practical Implementation for Why \& Why-Not Provenance (extended version)," 2018.
\bibitem{efficientSampling} Moshtaghi Largani, Sara, Lee, Seokki, "Efficient Sampling for Big Provenance," Companion Proceedings of the ACM Web Conference 2023, pp. 1508–1511, 2023.
\bibitem{c2d} Adnan Darwiche, "New advances in compiling CNF to decomposable negation normal form," Proceedings of ECAI, pp. 328--332, 2004.
\bibitem{provSQL} Senellart, Pierre, Jachiet, Louis, Maniu, Silviu, Ramusat, Yann, "ProvSQL: provenance and probability management in postgreSQL," Proc. VLDB Endow., vol. 11, no. 12, pp. 2034–2037, 2018.
\bibitem{dalvi2013dichotomy} Nilesh Dalvi, Dan Suciu, "The dichotomy of probabilistic inference for unions of conjunctive queries," Journal of the ACM (JACM), vol. 59, no. 6, pp. 1--87, 2013.
\bibitem{shapleyNegation} Reshef, Alon, Kimelfeld, Benny, Livshits, Ester, "The Impact of Negation on the Complexity of the Shapley Value in Conjunctive Queries," Proceedings of the 39th ACM SIGMOD-SIGACT-SIGAI Symposium on Principles of Database Systems, pp. 285–297, 2020.
\bibitem{shapley} Lloyd S. Shapley, "A value for n-person games," Contributions to the Theory of Games, vol. 2, no. 28, pp. 307--317, 1953.
\bibitem{fixpoint} Esparza, Javier, Luttenberger, Michael, "Solving fixed-point equations by derivation tree analysis," Proceedings of the 4th International Conference on Algebra and Coalgebra in Computer Science, pp. 19–35, 2011.
\bibitem{circuit} Daniel Deutch, Tova Milo, Sudeepa Roy, Val Tannen, "Circuits for Datalog Provenance," International Conference on Database Theory, 2014.
\bibitem{WhyAndWhyNot} Lee, Seokki, Lud\"{a}scher, Bertram, Glavic, Boris, "Approximate summaries for why and why-not provenance," Proc. VLDB Endow., vol. 13, no. 6, pp. 912–924, 2020.
\bibitem{dtree} Fink, Robert, Huang, Jiewen, Olteanu, Dan, "Anytime approximation in probabilistic databases," The VLDB journal, vol. 22, pp. 823--848, 2013.
\bibitem{elgebaly2014interpretable} Karim El Gebaly, Pankaj Agrawal, Lukasz Golab, Fan Korn, Divesh Srivastava, "Interpretable and informative explanations of outcomes," Proceedings of the VLDB Endowment (PVLDB), vol. 8, no. 1, pp. 61--72, 2014.
\bibitem{banzhaf} John F. Banzhaf III, "Weighted Voting Doesn't Work: A Mathematical Analysis," Rutgers Law Review, vol. 19, pp. 317--343, 1965.
\bibitem{castro2018} Javier Castro, Daniel Gómez, Elisenda Molina, Juan Tejada, "Improving polynomial estimation of the Shapley value by stratified random sampling with optimum allocation," Computers \& Operations Research, vol. 82, pp. 180-188, 2017.
\bibitem{maleki2014} Sasan Maleki, Long Tran-Thanh, Greg Hines, Talal Rahwan, Alex Rogers, "Bounding the Estimation Error of Sampling-based Shapley Value Approximation," 2014.
\bibitem{prox} Ainy, Eleanor, Bourhis, Pierre, Davidson, Susan B., Deutch, Daniel, Milo, Tova, "Approximated Summarization of Data Provenance," Proceedings of the 24th ACM International on Conference on Information and Knowledge Management, pp. 483–492, 2015.
\bibitem{gprom} Arab, Bahareh Sadat, Feng, Su, Glavic, Boris, Lee, Seokki, Niu, Xing, Zeng, Qitian, "GProM-a swiss army knife for your provenance needs," A Quarterly bulletin of the Computer Society of the IEEE Technical Committee on Data Engineering, vol. 41, no. 1, 2018.
\bibitem{spm} Floris Geerts, Thomas Unger, Grigoris Karvounarakis, Irini Fundulaki, Vassilis Christophides, "Algebraic Structures for Capturing the Provenance of {SPARQL} Queries," Journal of the ACM (JACM), vol. 63, no. 1, pp. 7:1--7:63, 2016.
\bibitem{sparQL} Hern\'{a}ndez, Daniel, Gal\'{a}rraga, Luis, Hose, Katja, "Computing how-provenance for SPARQL queries via query rewriting," Proc. VLDB Endow., vol. 14, no. 13, pp. 3389–3401, 2021.
\bibitem{headDom} Benny Kimelfeld, Jan Vondr\'{a}k, Ryan Williams, "Maximizing conjunctive views in deletion propagation," ACM Transactions on Database Systems (TODS), vol. 37, no. 4, pp. 1--37, 2012.
\bibitem{bernstein} Rémi Bardenet, Odalric-Ambrym Maillard, "Concentration inequalities for sampling without replacement," Bernoulli, vol. 21, no. 3, pp. 1361--1385, 2015.
\bibitem{neyman} Jerzy Neyman, "On the two different aspects of the representative method: the method of stratified sampling and the method of purposive selection," Breakthroughs in Statistics, pp. 123--150, 1992.
\bibitem{shapleySampling} Zhang, Jiayao, Sun, Qiheng, Liu, Jinfei, Xiong, Li, Pei, Jian, Ren, Kui, "Efficient Sampling Approaches to Shapley Value Approximation," Proc. ACM Manag. Data, vol. 1, no. 1, 2023.
\bibitem{senellart2018provsql} Senellart, Pierre, Jachiet, Louis, Maniu, Silviu, Ramusat, Yann, "Provsql: Provenance and probability management in postgresql," Proceedings of the VLDB Endowment (PVLDB), vol. 11, no. 12, pp. 2034--2037, 2018.
\bibitem{glavic2009perm} Glavic, Boris, Alonso, Gustavo, "Perm: Processing provenance and data on the same data model through query rewriting," 2009 IEEE 25th International Conference on Data Engineering, pp. 174--185, 2009.
\bibitem{castro2009polynomial} Castro, Javier, G{\'o}mez, Daniel, Tejada, Juan, "Polynomial calculation of the Shapley value based on sampling," Computers \& operations research, vol. 36, no. 5, pp. 1726--1730, 2009.
\bibitem{castro2017improving} Castro, Javier, G{\'o}mez, Daniel, Molina, Elisenda, Tejada, Juan, "Improving polynomial estimation of the Shapley value by stratified random sampling with optimum allocation," Computers \& Operations Research, vol. 82, pp. 180--188, 2017.
\bibitem{mitchell2022sampling} Mitchell, Rory, Cooper, Joshua, Frank, Eibe, Holmes, Geoffrey, "Sampling permutations for shapley value estimation," Journal of Machine Learning Research, vol. 23, no. 43, pp. 1--46, 2022.
\bibitem{burgess2021approximating} Burgess, Mark Alexander, Chapman, Archie C, "Approximating the Shapley Value Using Stratified Empirical Bernstein Sampling.," IJCAI, pp. 73--81, 2021.
\bibitem{zhang2023efficient} Zhang, Jiayao, Sun, Qiheng, Liu, Jinfei, Xiong, Li, Pei, Jian, Ren, Kui, "Efficient sampling approaches to shapley value approximation," Proceedings of the ACM on Management of Data, vol. 1, no. 1, pp. 1--24, 2023.
\bibitem{deng1994complexity} Deng, Xiaotie, Papadimitriou, Christos H, "On the complexity of cooperative solution concepts," Mathematics of operations research, vol. 19, no. 2, pp. 257--266, 1994.
\bibitem{faigle1992shapley} Faigle, Ulrich, Kern, Walter, "The Shapley value for cooperative games under precedence constraints," International Journal of Game Theory, vol. 21, pp. 249--266, 1992.
\bibitem{mann1960values} Mann, Irwin, Shapley, Lloyd S, "Values of large games, IV: Evaluating the electoral college by Montecarlo techniques," Rand Corporation, 1960.
\bibitem{owen1972multilinear} Owen, Guillermo, "Multilinear extensions of games," Management Science, vol. 18, no. 5-part-2, pp. 64--79, 1972.
\bibitem{liben2012computing} Liben-Nowell, David, Sharp, Alexa, Wexler, Tom, Woods, Kevin, "Computing shapley value in supermodular coalitional games," Computing and Combinatorics: 18th Annual International Conference, COCOON 2012, Sydney, Australia, August 20-22, 2012. Proceedings 18, pp. 568--579, 2012.
\bibitem{ando2012computation} Ando, Kazutoshi, "Computation of the Shapley value of minimum cost spanning tree games:\# P-hardness and polynomial cases," Japan Journal of Industrial and Applied Mathematics, vol. 29, no. 3, pp. 385--400, 2012.
\bibitem{banzhaf1965weighted} Banzhaf, John F, "Weighted voting doesn't work: A mathematical analysis," Rutgers Law Review, vol. 19, no. 2, pp. 317--343, 1965.
\bibitem{owen1977values} Owen, Guillermo, "Values of games with a priori unions," Essays in Mathematical Economics and Game Theory, pp. 76--88, 1977.
\bibitem{lundberg2017unified} Lundberg, Scott M, Lee, Su-In, "A unified approach to interpreting model predictions," Advances in Neural Information Processing Systems (NeurIPS), vol. 30, pp. 4765--4774, 2017.
\bibitem{fatima2008linear} Fatima, Shaheen S, Wooldridge, Michael, Jennings, Nicholas R, "A linear approximation method for the Shapley value," Artificial Intelligence, vol. 172, no. 14, pp. 1673--1699, 2008.
\bibitem{cochran1977} Cochran, William G., "Sampling Techniques," John Wiley \& Sons, 1977.
\bibitem{neyman1934} Neyman, Jerzy, "On the two different aspects of the representative method: The method of stratified sampling and the method of purposive selection," Journal of the Royal Statistical Society, vol. 97, no. 4, pp. 558--625, 1934.
\bibitem{etore2010adaptive} Étoré, Pierre, Jourdain, Benjamin, "Adaptive Optimal Allocation in Stratified Sampling Methods," Methodology and Computing in Applied Probability, vol. 12, pp. 335--360, 2010.
\bibitem{glynn1992} Glynn, Peter W, Whitt, Ward, "The asymptotic efficiency of simulation estimators," Operations Research, vol. 40, no. 3, pp. 505--520, 1992.
\bibitem{chalkiadakis2011computational} Chalkiadakis, Georgios, Elkind, Edith, Wooldridge, Michael, "Computational Aspects of Cooperative Game Theory," Morgan \& Claypool, 2011.
\bibitem{datta2016algorithmic} Datta, Anupam, Sen, Shayak, Zick, Yair, "Algorithmic transparency via quantitative input influence: Theory and experiments with learning systems," IEEE Symposium on Security and Privacy, pp. 598--617, 2016.
\bibitem{wang2019database} Wang, Ying, Cheney, James, "Database Causal Analysis: Abductive Reasoning with Data Provenance," Proceedings of the 38th ACM SIGMOD-SIGACT-SIGAI Symposium on Principles of Database Systems (PODS), 2019.
\bibitem{gogate2019provenance} Gogate, Nevin, Olteanu, Dan, Vagena, Zografoula, "Provenance Summarization for Aggregation Queries," Proceedings of the VLDB Endowment, vol. 12, no. 12, pp. 1910--1923, 2019.
\bibitem{koutris2016query} Koutris, Paraschos, Olteanu, Dan, "Query-based Decision Provenance and Explanation," Proceedings of the 19th International Conference on Database Theory (ICDT), 2016.
\bibitem{chen2022cleaning} Chen, Zeyuan, Yin, Xiaolan, Wu, Eugene, Roy, Sudeepa, "Cleaning by Attribution," Proceedings of the 2022 ACM SIGMOD International Conference on Management of Data, pp. 67--80, 2022.
\bibitem{maleki2013bounding} Maleki, Sattar, Ostadabbas, Sareh, Ghosh, Arpita, "Bounding the Estimation Error of Sampling-Based Shapley Value Approximation," Advances in Neural Information Processing Systems, vol. 26, 2013.
\bibitem{amarilli2021provenance} Amarilli, Antoine, Monet, Mikaël, "Acyclic Conjunctive Queries and Shapley-based Query Explanation," ACM Transactions on Database Systems (TODS), vol. 46, no. 3, pp. 1--42, 2021.
\end{thebibliography}

